ROGLE: Robust Global-Local Alignment with Automated Region Supervision for Text-Based Person Search

Text-Based Person Search (TBPS) aims to retrieve pedestrian images using natural language queries. However, existing TBPS models, especially those based on CLIP, struggle with fine-grained understanding due to global representational bias and semantic sparsity inherited from training on short captions. This results in weak fine-grained alignment, exacerbated by the scarcity of region-level annotations. To address this, we propose ROGLE (Robust Global-Local Embedding), a unified framework that overcomes reliance on costly manual annotations through an automated Region-to-Sentence Matching (RSM) strategy. RSM automatically mines pseudo region-sentence pairs for scalable fine-grained supervision. Furthermore, ROGLE employs a multi-granular learning strategy that fuses global contrastive learning with region-level local alignment. We also introduce the P-VLG Benchmark, a large-scale dataset constructed by curating and enriching images from established public benchmarks. It features over 100,000 annotated regions and rich long-form captions, making it the first TBPS benchmark to support both global and local assessment protocols. Extensive experiments show that ROGLE significantly outperforms existing approaches, particularly on challenging long-form queries. Code and the P-VLG benchmark will be made publicly available.

==> sec/3_method1.tex <==
\section{Method}
\label{sec:method}





\subsection{Region-to-Sentence Matching (RSM)}
\label{subsec:rsm}




Both visual and textual inputs are then encoded using the CLIP model. Each image patch $\mathcal{I}_l^{(i)}$ and sentence $\mathcal{T}_l^{(j)}$ is passed through the CLIP image encoder $f^{\mathcal{I}}$ and text encoder $f^{\mathcal{T}}$, respectively:
\[
\boldsymbol{i}_l^{(i)} = f^{\mathcal{I}}(\mathcal{I}_l^{(i)}), \quad \boldsymbol{t}_l^{(j)} = f^{\mathcal{T}}(\mathcal{T}_l^{(j)}).
\]
For reference, we also extract global features from the full image and full caption:
\[
\boldsymbol{i}_g = f^{\mathcal{I}}(\mathcal{I}_g), \quad \boldsymbol{t}_g = f^{\mathcal{T}}(\mathcal{T}_g).
\]

Cosine similarity is computed between all region–sentence pairs, and the highest-scoring pair is selected:
\[
(i^*, j^*) = \arg\max_{i, j} \cos\left( \boldsymbol{i}_l^{(i)}, \boldsymbol{t}_l^{(j)} \right).
\]
If the selected region $\mathcal{I}_l^{(i^*)}$ covers the entire image, the pair is discarded to retain locality. The remaining top-aligned pair $(\mathcal{I}_l, \mathcal{T}_l) = (\mathcal{I}_l^{(i^*)}, \mathcal{T}_l^{(j^*)})$ is then used as a pseudo-local supervision sample in the collaborative learning stage.

\subsection{Global–Local Collaborative Learning}
\label{subsec:collab}

Given both global $(\mathcal{I}_g, \mathcal{T}_g)$ and local $(\mathcal{I}_l, \mathcal{T}_l)$ pseudo-pairs, we adopt a unified learning strategy that combines contrastive supervision with token-level alignment. Global image and text inputs are encoded with CLIP to yield global-level [CLS] features $\boldsymbol{i}_g = f^\mathcal{I}(\mathcal{I}_g)$ and $\boldsymbol{t}_g = f^\mathcal{T}(\mathcal{T}_g)$, while the local pair yields $\boldsymbol{i}_l = f^\mathcal{I}(\mathcal{I}_l)$ and $\boldsymbol{t}_l = f^\mathcal{T}(\mathcal{T}_l)$.

To enable fine-grained understanding, we also extract token-level features from the full caption and image:
\[
\boldsymbol{S}_g = f^{\mathcal{T}}(\mathcal{T}_g) \in \mathbb{R}^{M \times d}, \quad
\boldsymbol{P}_g = f^{\mathcal{I}}(\mathcal{I}_g) \in \mathbb{R}^{N \times d}.
\]
Using index sets $\mathcal{T}$ and $\mathcal{B}$ that map the local text $\mathcal{T}_l$ and region $\mathcal{I}_l$ to their positions in global sequences, we compute contextual span representations by averaging the corresponding tokens. These are projected into a shared space via a learnable layer:
\[
\tilde{\boldsymbol{t}}_l = \text{proj} \left( \frac{1}{|\mathcal{T}|} \sum_{k \in \mathcal{T}} \boldsymbol{S}_g[k] \right), \quad
\tilde{\boldsymbol{i}}_l = \text{proj} \left( \frac{1}{|\mathcal{B}|} \sum_{k \in \mathcal{B}} \boldsymbol{P}_g[k] \right).
\]

To jointly train both global and local branches, we define the total loss as:
\[
\mathcal{L}_{\text{total}} = \lambda_g \mathcal{L}_{\text{global}} + \lambda_l \mathcal{L}_{\text{local}} + \lambda_{\text{tok}} \mathcal{L}_{\text{token}},
\]
where $\mathcal{L}_{\text{global}} = \mathcal{L}_{\text{contrast}}(\boldsymbol{i}_g, \boldsymbol{t}_g)$ ensures coarse alignment, $\mathcal{L}_{\text{local}} = \mathcal{L}_{\text{contrast}}(\boldsymbol{i}_l, \boldsymbol{t}_l)$ promotes detailed matching, and the token-level loss is defined as:
\[
\mathcal{L}_{\text{token}} = \text{MSE}(\text{sim}(\tilde{\boldsymbol{t}}_l, \boldsymbol{t}_l), 1) + \text{MSE}(\text{sim}(\tilde{\boldsymbol{i}}_l, \boldsymbol{i}_l), 1),
\]
where $\text{sim}(\cdot,\cdot)$ denotes cosine similarity and MSE is the mean squared error. This encourages alignment between pooled token representations and their corresponding [CLS] features. The hyperparameters $\lambda_g$, $\lambda_l$, and $\lambda_{\text{tok}}$ control the balance between each component.

\subsection{Training Objective}

To optimize both global and local alignment, we formulate a three-part loss function combining global contrastive loss, local contrastive loss, and token-level alignment. The overall loss is:

\begin{equation}
\mathcal{L}_{\text{total}} = \lambda_g \mathcal{L}_{\text{global}} + \lambda_l \mathcal{L}_{\text{local}} + \lambda_{\text{tok}} \mathcal{L}_{\text{token}},
\end{equation}

with scalar weights $\lambda_g$, $\lambda_l$, and $\lambda_{\text{tok}}$.

The global loss promotes semantic consistency between the full image and caption:

\begin{equation}
\mathcal{L}_{\text{global}} = \mathcal{L}_{\text{contrast}}(\boldsymbol{i}_g, \boldsymbol{t}_g).
\end{equation}

The local loss encourages fine-grained alignment between the region and sentence:

\begin{equation}
\mathcal{L}_{\text{local}} = \mathcal{L}_{\text{contrast}}(\boldsymbol{i}_l, \boldsymbol{t}_l).
\end{equation}

The token-level term refines alignment between token-aggregated spans and their global embeddings:

\begin{equation}
\mathcal{L}_{\text{token}} = \text{MSE}(\text{sim}(\tilde{\boldsymbol{t}}_l, \boldsymbol{t}_l), 1) + \text{MSE}(\text{sim}(\tilde{\boldsymbol{i}}_l, \boldsymbol{i}_l), 1).
\end{equation}

This composite loss enables ROGLE to jointly optimize across multiple levels of semantic granularity, supporting robust fine-grained understanding in TBPS tasks.


==> table/tb5.tex <==
% \begin{table*}
% \caption{ Performance of methods and components in cross-domain tests.  CUHK-PEDES is abbreviated as CUHK, ICFG-PEDES as ICFG, and RSTPReid as RSTP. The arrow → indicates that the method was trained on the dataset on the left and tested on the dataset on the right. The best results are in bold.}
%   \label{tab:5}
% \begin{center}
% \scalebox{1.02}{
%    \begin{tabular}{c|c|ccc|c|ccc}
% \toprule
% \textbf{Method} & \textbf{Domain} & \textbf{R1} & \textbf{R5} & \textbf{mAP} & \textbf{Domain} & \textbf{R1} & \textbf{R5} & \textbf{mAP} \\
% % \midrule
% % \multirow{3}{*}{{IRRA} ~\cite{IRRA} }
% %  & CUHK $\rightarrow$ RSTP & 53.30 & 77.15 & 39.63 & CUHK $\rightarrow$ ICFG & 42.42 & 62.11 & 21.77 \\
% %  & ICFG $\rightarrow$ RSTP & 45.30 & 69.35 & 36.83 & ICFG $\rightarrow$ CUHK & 33.46 & 56.30 & 31.56 \\
% %  & RSTP $\rightarrow$ ICFG & 32.30 & 49.69 & 20.54 & RSTP $\rightarrow$ CUHK & 32.80 & 55.25 & 30.29 \\
% % \midrule
% % \multirow{3}{*}{{SEN} ~\cite{liu2025textsen}} 
% %  & CUHK $\rightarrow$ RSTP & 55.50 & 77.85 & 45.29 & CUHK $\rightarrow$ ICFG & 45.34 & 63.45 & 23.26 \\
% %  & ICFG $\rightarrow$ RSTP & 47.45 & 71.95 & 39.86 & ICFG $\rightarrow$ CUHK & 37.88 & 60.48 & 35.07 \\
% %  & RSTP $\rightarrow$ ICFG & 36.23 & 53.31 & 22.32 & RSTP $\rightarrow$ CUHK & 35.40 & 57.71 & 33.41 \\

% \midrule
% \multirow{1}{*}{{ROGLE} (Ours)} 
%  % & CUHK $\rightarrow$ RSTP & 55.50 & 77.85 & 45.29 & CUHK $\rightarrow$ ICFG & 45.34 & 63.45 & 23.26 \\
%  % & ICFG $\rightarrow$ RSTP & 47.45 & 71.95 & 39.86 & ICFG $\rightarrow$ CUHK & 37.88 & 60.48 & 35.07 \\
%  & P-VLG $\rightarrow$ ICFG & 62.78 & 78.19 &  38.58
%  & P-VLG $\rightarrow$ CUHK & 47.74 & 68.65 & 43.10 \\
% \bottomrule
% \end{tabular}


% }
% \end{center}
% \end{table*}



\begin{table}
\caption{Performance of methods and components in cross-domain tests. CUHK-PEDES is abbreviated as CUHK, ICFG-PEDES as ICFG. The arrow → indicates that the method was trained on the dataset on the left and tested on the dataset on the right. The best results are in bold.}
\label{tab:5}
\begin{center}
\scalebox{1.0}{
   \begin{tabular}{c|c|ccc}
\toprule
\textbf{Method} & \textbf{Domain} & \textbf{R1} & \textbf{R5} & \textbf{mAP} \\
\midrule
\multirow{2}{*}{\textbf{ROGLE}} 
 & P-VLG $\rightarrow$ ICFG & \textbf{62.78} & \textbf{78.19} & \textbf{38.58} \\
 & P-VLG $\rightarrow$ CUHK & \textbf{47.74} & \textbf{68.65} & \textbf{43.10} \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}
